P-value evaluation, variability index and biomarker categorization for adaptively weighted Fisher's meta-analysis method in omics applications

Meta-analysis methods have been widely used to combine results from multiple clinical or genomic studies to increase statistical power and ensure robust and accurate conclusion. Adaptively weighted Fisher's method (AW-Fisher) is an effective approach to combine p-values from $K$ independent studies and to provide better biological interpretation by characterizing which studies contribute to meta-analysis. Currently, AW-Fisher suffers from lack of fast, accurate p-value computation and variability estimate of AW weights. When the number of studies $K$ is large, the $3^K - 1$ possible differential expression pattern categories can become intractable. In this paper, we apply an importance sampling technique with spline interpolation to increase accuracy and speed of p-value calculation. Using resampling techniques, we propose a variability index for the AW weight estimator and a co-membership matrix to characterize pattern similarities between genes. The co-membership matrix is further used to categorize differentially expressed genes based on their meta-patterns for further biological investigation. The superior performance of the proposed methods is shown in simulations. These methods are also applied to two real applications to demonstrate intriguing biological findings.

==> figure/biomarkerCategorization/tight_table.tex <==
1 & 0 & \textbf{177} & 0 & 0 & 0 & 0 & 0\\
2 & \textbf{184} & 0 & 0 & 0 & 0 & 0 & 0\\
3 & 0 & 0 & 0 & \textbf{74} & 0 & 0 & 1\\
4 & 0 & 0 & \textbf{60} & 0 & 0 & 0 & 1\\
5 & 0 & 0 & 0 & 0 & 0 & \textbf{102} & 2\\
6 & 0 & 0 & 0 & 0 & \textbf{85} & 0 & 3\\
0 & 13 & 24 & 19 & 11 & 6 & 5 & \textbf{27}\\


==> figure/simulation/accuracy/AW_CI_G_10000_N_50_K_2/close2.tex <==
NA & 3.43$ \sim $27.5 & NA & 0.0693 secs \\

==> figure/simulation/accuracy/AW_CI_G_10000_N_50_K_2/interpolation.tex <==
NA & 3.43$ \sim $27.5 & 0.107 & 0.0248 secs \\

==> figure/simulation/accuracy/AW_CI_G_10000_N_50_K_2/permutation_100.tex <==
100 & 3.43$ \sim $27.5 & 31.3 & 1.05 mins \\

==> figure/simulation/accuracy/AW_CI_G_10000_N_50_K_2/permutation_1000.tex <==
1000 & 3.43$ \sim $27.5 & 30.6 & 10.1 mins \\

==> figure/simulation/accuracy/AW_CI_G_10000_N_50_K_2/permutation_10000.tex <==
10000 & 3.43$ \sim $27.5 & 30 & 2.83 hours \\

==> figure/simulationRes/varibility100.tex <==
0.00132 (0.00017) & 0.0084 (0.00041) & 0.0251 (7e-04) & 0.0456 (0.00089)\\


==> figure/simulationRes/varibility20.tex <==
0.0103 (0.00045) & 0.0512 (0.00093) & 0.0926 (0.0011) & 0.127 (0.0011)\\


==> figure/simulationRes/varibility50.tex <==
0.00365 (0.00027) & 0.0209 (0.00064) & 0.0472 (9e-04) & 0.0767 (0.001)\\

